Constructing the Virasoro groups using differential cohomology

The Virasoro groups are a family of central extensions of $\mathrm{Diff}^+(S^1)$, the group of orientation-preserving diffeomorphisms of $S^1$, by the circle group $\mathbb T$. We give a novel, geometric construction of these central extensions using "off-diagonal" differential lifts of the first Pontryagin class, thus affirmatively answering a question of Freed-Hopkins.

==> outtakes.tex <==
% Outtake from Section 5: Picking coordinates
We set explicit coordinates for this
action. Let $\theta$ be the $1$-periodic coordinate for $S^1$; that is, $\theta$ identifies $S^1$ with $\R/\Z$.
Give the frame bundle $F\cong\R^+\times S^1$ the coordinates $(v, \theta)$, and give $\R$ the coordinate $x$.
We will let $\gamma$ be an element of $\Gamma$, and think of it as a map $\gamma:\R \to \R$ satisfying
\begin{equation}
	\gamma(\theta + 1) = \gamma(\theta) + 1.
\end{equation}
The left $\Gamma$-action and right $\R$-action on $F$ are given by
\begin{subequations}
\begin{align}
    \gamma \cdot (v, \theta) &= (\gamma'(\theta) \cdot  v, \gamma(\theta))\\
	(v, \theta) \cdot x &= (e^x \cdot v, \theta).
\end{align}
\end{subequations}

% BIG outtake from main_statement.tex
%\TODO: QED here?
%\end{proof} 
 %%%%%%%%%%%%%%%% Rewrite below %%%%%%%%%%%%%%
 \newpage
 We begin by reducing the computation to differential forms. There is a map of sheaves $\Omega^{-1}[-2] \rightarrow \Z(2)$. Functoriality of pullback and integration imply the following commutative diagram:
 \begin{equation}
 \begin{tikzcd} \label{reduction-to-diff-form}
     H^2(\Bdot\R,\Omega^1) \ar[r,"q^\ast"] \ar[d] &
     H^2(\Gamma \backslash S^1, \Omega^1) \ar[r,"{\int_{S_1}}"] \ar[d] &
     H^2(\Bdot \Gamma,\Omega^0) \ar[d] \\
     H^4(\Bdot\R,\Z(2)) \ar[r,"q^\ast"] &
     H^4(\Gamma \backslash S^1, \Z(2)) \ar[r,"{\int_{S_1}}"] &
     H^3(\Bdot \Gamma,\Z(1)) 
 \end{tikzcd}
 \end{equation}

 Recall that $\Z(1)[1] \simeq \T$, thus $H^3(\Bdot \Gamma, \Z(1)) \simeq H^2(\Bdot \Gamma, \T)$. The composition is given by 
 \begin{equation}
     \exp(2\pi \ii - ): \Omega^0 \to \Z(1)[1] \to \underline\T.
 \end{equation}

 For $G = \R$, all $H^4(\Bdot\R, \Z(2))$ cohomology classes come from differential forms:
 \begin{lem}
 \label{pullback_to_diff_forms}
 Recall $G=\R$, the additive group of reals.
 The map
     \begin{equation}
         H^2(\Bdot\R, \Omega^1) \to H^4(\Bdot\R, \Z(2))
     \end{equation}
     induced by the inclusion of sheaves
     \begin{equation}
         \Omega^1[-2] \to \Z(2) 
     \end{equation}
     is an isomorphism.
 \end{lem}
 \begin{proof}
     First, note $H^k(\Bdot\R,\Z(1))=0$ for $k > 2$. 
     This follows from 
     \begin{align*}
         H^k(\Bdot\R,\Z)=H^k(BG,\Z)=H^k(\point,\Z)\overset{k>0}{=} 0, \\
         H^k(\Bdot\R,\Omega^0)=H^k_{\Lie}(\mathfrak{g},\R) \iso H^k_{\Lie}(\R,\R)\overset{k>1}{=}0,
     \end{align*}
     and the long exact sequence
     \begin{equation}
         \cdots \to H^k(\Bdot\R, \Omega^0) \to H^{k+1}(\Bdot\R, \Z(1)) \to 
         H^{k+1}(\Bdot\R,\Z) \to H^{k+1}(\Bdot\R,\Omega^0) \to \cdots.
     \end{equation}
   
     Now consider the exact sequence $\Omega^1[-2] \to \Z(2) \to \Z(1)$.
     Together with $H^3(\Bdot\R,\Z(1))=H^4(\Bdot\R,\Z(1))=0$, 
     the associated long exact sequence
 %    \begin{equation}
 %        \cdots \to H^{k-1}(\Bdot\R, \underline\T) \to 
 %        H^k(\Bdot\R, \Omega^1[-1]) \to H^k(\Bdot\R,\underline\T(1)) 
 %        \to H^k(\Bdot\R,\underline\T) \to \cdots
 %    \end{equation}
     gives an isomorphism
     \begin{equation}
         H^2(\Bdot\R, \Omega^1) = H^4(\Bdot\R,\Omega^1[-2]) \isoto H^4(\Bdot\R,\Z(2)).
     \end{equation}
 \end{proof}

 Therefore we can work with the top line of Diagram~\ref{reduction-to-diff-form}.  
 Note that $H^2(\Bdot \Gamma, \R) \rightarrow H^2(\Bdot H, \T)$ takes a central extension of $\Gamma$ by $\R$ 
 to a central extension of $\Gamma$ by $\T$, as described in \cref{vira-from-R-extension}. 
 %Since the Virasoro family $\tGam_\lambda$ also comes from $\R$ central extension, 
 %we are reduced to the following proposition:
 \begin{prop}
     The transgression map 
     $\int_{S_1} \circ \ q^\ast: H^2(\Bdot\R,\Omega^1) \to H^2(\Bdot\Gamma,\Omega^0)$ maps
     to the extensions $\underline\R \to \GpVir_\R \to \Gamma$
     with representing cocycle proportional to\TODO: different name for cocycle
     \begin{align}
  (\gamma_1,\gamma_2) &\mapsto -\int_{S^1} \log(\gamma_1'\circ\gamma_2) \ud(\log(\gamma_2))'.
     \end{align}
 \end{prop}

 %\begin{proof}
 We compute the map explicitly on cocycles, using simplicial presentations of the spaces involved.
 $\Bdot\R$ admits a presentation by the simplicial manifold 
 \begin{equation}
 \begin{tikzcd}
 	\point & 
 	\ar[l,shift left=0.1em] \ar[l,shift right=0.1em]  \R &
 	\ar[l,shift left=0.2em] \ar[l] \ar[l,shift right=0.2em] \R\times \R &
 	\ar[l,shift left=0.3em] \ar[l,shift left=0.1em]
 	\ar[l,shift right=0.1em] \ar[l,shift right=0.3em] \R\times \R\times \R \cdots.
 \end{tikzcd}
 \end{equation}
 The sheaf $\Omega^1$ is soft, and thus acyclic on paracompact manifolds.
 As a result, the cochain complex $\Omega^1({\Bdot\R}_\bullet):$
     \begin{equation}
     \label{omegaOfBdotG}
         \begin{tikzcd}
 	        \Omega^1(\point)  
 	        \ar[r,shift left=0.1em]  \ar[r,shift right=0.1em]  & \Omega^1(\R) 
 	        \ar[r,shift left=0.2em]  \ar[r] \ar[r,shift right=0.2em] & \Omega^1(\R\times \R) 
 	        \ar[r,shift left=0.3em]  \ar[r,shift left=0.1em]
 	        \ar[r,shift right=0.1em] \ar[r,shift right=0.3em] &\Omega^1(\R\times \R\times \R) \dots,
         \end{tikzcd}
     \end{equation}
 computes the cohomology $H^*(\Bdot\R, \Omega^1)$. 
 The cohomology classes admit cocycle representatives which are globally defined 1-forms --- contrast
 this with the case of a general sheaf over $\Man$, where general cocycles over a simplicial manifold $Y_\bullet$ 
 only admit a representation as sections over a hypercover of $Y_\bullet$.
 \begin{lem}
     $H^2(\Bdot\R, \Omega^1)$ is generated by the class of the cocycle
 	\begin{equation}
     \begin{aligned}
         \omega_{\hat{p}_1}: \underline\R \times \underline\R &\to \Omega^1 \\
         (x_1, x_2) &\mapsto x_2 \ud x_1.
     \end{aligned}
 	\end{equation}
 \end{lem}

 \TODO: I (Christoph) think we should include at least a brief proof of this. (sth like the one commented out below)
 % \begin{proof}
 %     The group $H^2(\Bdot\R, \Omega^1)$ is isomorphic to $\R$ by \cref{pullback_to_diff_forms} and \cref{GLn_off_diag}.
 %     The sheaves $\Omega^i$ are soft on manifolds \TODO: reference,
 %     so $H^\ast(\Bdot\R,\Omega^i)$ is computed by the simplicial complex $\Omega^i(\Bdot\R)$:
 %     \begin{equation}
 %     \label{omegaOfBdotG}
 %         \begin{tikzcd}
 % 	        \Omega^i(\point)  
 % 	        \ar[r,shift left=0.1em]  \ar[r,shift right=0.1em]  & \Omega^i(G) 
 % 	        \ar[r,shift left=0.2em]  \ar[r] \ar[r,shift right=0.2em] & \Omega^i(G\times G) 
 % 	        \ar[r,shift left=0.3em]  \ar[r,shift left=0.1em]
 % 	        \ar[r,shift right=0.1em] \ar[r,shift right=0.3em] &\Omega^i(G\times G\times G) \dots,
 %         \end{tikzcd}
 %     \end{equation}
 %     and $k$-cocyles are those $1$-forms $\omega \in \Omega^i(G^k)$, whose alternating pullback to 
 %     $G^{k+1}$ vanishes.
 %     For $i=1, k=2$, it is straightforward to check that the 1-form
 %     $(x_1, x_2) \mapsto x_2 \d x_1$ is a cocycle, but not a coboundary in this complex.
 % \end{proof}

 Now we want to compute the pullback of the cocycle to $\GFR$. 
 We compute this with respect to the following simplicial presentation of the map 
 $\GFR \to \Bdot\R$:
 \begin{equation}
 \begin{tikzcd}
 	\ar[d] \GF & 
 	\ar[d] \ar[l,shift left=0.1em] \ar[l,shift right=0.1em]  \GF \times \R&
 	\ar[d] \ar[l,shift left=0.2em] \ar[l] \ar[l,shift right=0.2em] \GF\times \R \times \R &
 	\ar[d] \ar[l,shift left=0.3em] \ar[l,shift left=0.1em]
 	\ar[l,shift right=0.1em] \ar[l,shift right=0.3em] \GF\times \R\times \R \times \R \dots \\
 	\point & 
 	\ar[l,shift left=0.1em] \ar[l,shift right=0.1em]  \R &
 	\ar[l,shift left=0.2em] \ar[l] \ar[l,shift right=0.2em] \R\times \R &
 	\ar[l,shift left=0.3em] \ar[l,shift left=0.1em]
 	\ar[l,shift right=0.1em] \ar[l,shift right=0.3em] \R\times \R\times \R \dots
 \end{tikzcd}
 \end{equation}
 where the vertical maps simply forget the first factor.
 The pullback map $p^*: \Omega^1(\Bdot\R) \rightarrow 
 \Omega^1((\Gamma \backslash \F)/\R_\bullet)$ sends the cocycle $x_2 dx_1 \in
 \Omega^1(\R^2)$ to $x_2 dx_1 \in \Omega^1(\Gamma \backslash \F) \times \R^2$. 

 While the simplicial presentation above makes the computation of the pullback trivial, 
 it is less suitable for studying integration over $S^1$. 
 There is another model for $\GFR$ which simplifies the description of the pushforward
 $\int_{S^1}$, given by the simplicial Fr\'echet manifold $\Gamma \backslash (F/\R)_\bullet$:
 \begin{equation}
 \begin{tikzcd}
 	F/\R & 
 	\ar[l,shift left=0.1em] \ar[l,shift right=0.1em]  \Gamma \times F/\R &
 	\ar[l,shift left=0.2em] \ar[l] \ar[l,shift right=0.2em] \Gamma \times \Gamma \times F/\R &
 	\ar[l,shift left=0.3em] \ar[l,shift left=0.1em]
 	\ar[l,shift right=0.1em] \ar[l,shift right=0.3em] \Gamma \times \Gamma \times \Gamma \dots F/\R.
 \end{tikzcd}
 \end{equation}

 The map $q: \GFR \rightarrow \Bdot \Gamma$ admits a presentation by a simplicial map
 \begin{equation}
 \begin{tikzcd}
 	\dar F/\R & 
 	\dar \ar[l,shift left=0.1em] \ar[l,shift right=0.1em]  \Gamma \times F/\R &
 	\dar \ar[l,shift left=0.2em] \ar[l] \ar[l,shift right=0.2em] \Gamma \times \Gamma \times F/\R &
 	\dar \ar[l,shift left=0.3em] \ar[l,shift left=0.1em]
 	\ar[l,shift right=0.1em] \ar[l,shift right=0.3em] \Gamma \times \Gamma \times \Gamma  F/\R \dots. \\
 	\point & 
 	\ar[l,shift left=0.1em] \ar[l,shift right=0.1em]  \Gamma &
 	\ar[l,shift left=0.2em] \ar[l] \ar[l,shift right=0.2em] \Gamma\times \Gamma &
 	\ar[l,shift left=0.3em] \ar[l,shift left=0.1em]
 	\ar[l,shift right=0.1em] \ar[l,shift right=0.3em] \Gamma\times \Gamma\times \Gamma \dots
 \end{tikzcd}
 \end{equation}
 which is a level-wise $S^1$-fibration.
 Thus $p_*: \Omega^1(\Gamma \backslash (F/\R)_\bullet) \rightarrow
 \Omega^1(\Bdot\Gamma)$ is simply given by integration over $S^1$.

 To get the cocycle from one to another, we use the bisimplicial presentation  $\GFR_{\bullet,\bullet}$ with 
 $\GFR_{p,q} = \Gamma^p \times F \times \R^q$:
 \begin{equation}
 \begin{gathered}
 \begin{tikzcd}[column sep=3em,row sep=3em]
     &
 	\cdots
 	\ar[d,shift left=0.3em]  \ar[d,shift left=0.1em]
 	\ar[d,shift right=0.1em] \ar[d,shift right=0.3em] &
 	\cdots
 	\ar[d,shift left=0.3em]  \ar[d,shift left=0.1em]
 	\ar[d,shift right=0.1em] \ar[d,shift right=0.3em] &
 	\cdots
 	\ar[d,shift left=0.3em]  \ar[d,shift left=0.1em]
 	\ar[d,shift right=0.1em] \ar[d,shift right=0.3em] 
 	\\
     \cdots
 	\ar[r,shift left=0.3em]  \ar[r,shift left=0.1em]
 	\ar[r,shift right=0.1em] \ar[r,shift right=0.3em] &
 	\Gamma^{\times 2} \times F \times \R^{\times 2}
 	\ar[d,shift left=0.2em]  \ar[d] \ar[d,shift right=0.2em]
 	\ar[r,shift left=0.2em]  \ar[r] \ar[r,shift right=0.2em] &
     \Gamma \times F \times \R^{\times 2}
 	\ar[d,shift left=0.2em]  \ar[d] \ar[d,shift right=0.2em]
 	\ar[r,shift left=0.1em]  \ar[r,shift right=0.1em] &
 	F \times \R^{\times 2}
 	\ar[d,shift left=0.2em]  \ar[d] \ar[d,shift right=0.2em]
 	\\
     \cdots
 	\ar[r,shift left=0.3em]  \ar[r,shift left=0.1em]
 	\ar[r,shift right=0.1em] \ar[r,shift right=0.3em] &
 	\Gamma^{\times 2} \times F \times \R
 	\ar[d,shift left=0.1em]  \ar[d,shift right=0.1em]
 	\ar[r,shift left=0.2em]  \ar[r] \ar[r,shift right=0.2em] &
     \Gamma \times F \times \R
 	\ar[d,shift left=0.1em]  \ar[d,shift right=0.1em]
 	\ar[r,shift left=0.1em]  \ar[r,shift right=0.1em] &
 	F \times \R
 	\ar[d,shift left=0.1em]  \ar[d,shift right=0.1em]
 	\\
     \cdots
 	\ar[r,shift left=0.3em]  \ar[r,shift left=0.1em]
 	\ar[r,shift right=0.1em] \ar[r,shift right=0.3em] &
 	\Gamma^{\times 2} \times F
 	\ar[r,shift left=0.2em]  \ar[r] \ar[r,shift right=0.2em] &
     \Gamma \times F 
 	\ar[r,shift left=0.1em]  \ar[r,shift right=0.1em] &
 	F 
 \end{tikzcd}
 \end{gathered}
 \end{equation}
 %\end{proof}
 The bisimplicial complex $\Omega^1(\GFR_{\bullet,\bullet})$ intertwines between the two above-mentioned complexes 
 \begin{equation}
 \begin{tikzcd}
 \Omega^1(\GFR_{\bullet, \bullet})
 & \arrow[l, "f^*"] \Omega^1(((\Gamma \backslash F)/\R)_\bullet)  \\
 \Omega^1({\Gamma \backslash (F/\R)}_\bullet) \arrow[u, "g^*"].
 & 
 \end{tikzcd}
 \end{equation}
 The total complex in degree 3 is 
 \begin{equation}
     \Omega^1(F \times \R^{\times 2}) \oplus \Omega^1(\Gamma \times F \times \R) \oplus 
     \Omega^1(\Gamma^{\times 2} \times F)
 \end{equation}
 $a (x_2 dx_1) = (x_2 dx_1, 0, 0)$, and the cocycle we want is $(0,0, -\log(\gamma_1'\circ\gamma_2) \ud(\log(\gamma_2)))$. Therefore it is suffice to show that they are cohomologous:
 \TODO: if the minus is here, it shouldn't be in the Lemma below! $d\beta$ should be the difference of the 
 two cocycles
 \begin{lem}\label{main_lemma} The two cocycles are cohomologous:
 \begin{equation}
     (x_2 dx_1, 0, -\log(\gamma_1'\circ\gamma_2) \ud(\log(\gamma_2))) = d \beta
 \end{equation}
 where $\beta = (\log(v)\ud\log(\gamma'), x \ud\log(v))$ is a  $2$-form in the double complex, with
 $\log(v)\ud\log(\gamma') \in \Omega^1(\Gamma \times F)$ and $x\ud\log(v) \in \Omega^1(F \times \R)$.
 \end{lem}
 \begin{proof}
 We provide a visualisation of the computation.
 \TODO: maybe insert a part of the computation from computations.tex
 \begin{equation}
 \begin{tikzpicture}
     \draw  node (N20) at (-6,0) {$\Omega^1(\Gamma^{\times 2} \times F)$}
           node (N10) at (-3,0) {$\Omega^1(\Gamma \times F)$}
           node (N11) at (-3,3) {$\Omega^1(\Gamma \times F \times \R)$}
           node (N01) at (0,3)  {$\Omega^1(F \times \R)$}
           node (N02) at (0,6)  {$\Omega^1(F \times \R^{\times 2})$};
     \draw [->] (N10) -- (N20);
     \draw [->] (N10) -- (N11);
     \draw [->] (N01) -- (N11);
     \draw [->] (N01) -- (N02);
     \begin{scope}[shift={(1,-0.5)}]
         \draw  node (C20) at (-6,0) {$x_2 \d x_1$} 
               node (C10) at (-3,0) {$x\ \ud\log(v)$}
               node (C11) at (-3,3) 
               [align=center]{\\
               $\textcolor{blue}{x \log \gamma^\prime} -$ \\
               $\textcolor{red}{x \log \gamma^\prime} = 0$}
               node (C01) at (0,3)  {$\log(v)\ \ud\log(\gamma^\prime)$}
               node (C02) at (0,6)  {\hspace{5em}
               $-\log(\gamma_1'\circ\gamma_2) \ud\log(\gamma_2)$};
         \draw [|->] (C10) -- (C20);
         \draw [|->,draw=red] (C10) -- (C11);
         \draw [|->,draw=blue] (C01) -- (C11);
         \draw [|->] (C01) -- (C02);
     \end{scope}
 \end{tikzpicture}
 \end{equation}
 \end{proof}

We need to show that the horizontal and vertical differentials of the $log\ v \ d\ log \gamma'$ is $\alpha$ and $x\ log\ \gamma$, and the horizontal and vertical differentials of $x \ d\ log\ v$ is $x \log \gamma$ and $x_2 \ dx_1$. (\TODO: proof the lemma somewhere.). 

 \newpage
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 We have coordinates: the coordinate on $\mb{R}$ is $x$, the coordinates on $F = \mb{R}^{>0} \times S^1$ is $v, \theta$, the coordinate on $\Gamma$ is $\gamma$. $x$ acts on $F$ as
 \begin{equation}
     (v, \theta) \mapsto (e^x v, \theta)
 \end{equation}
 and $\gamma$ acts on $F$ as 
 \begin{equation}
     (v, \theta) \mapsto (\gamma'(\theta) v, \gamma(\theta))
 \end{equation}
 
 We will compute the transgression map by proceeding along the bottom row 
 of the commutative diagram below.
 \begin{equation}
 \begin{tikzcd}
     H^4(\Bdot\R,\Z(2)) \ar[r,"q^\ast"] &
     H^4(\Gamma \backslash S^1, \Z(2)) \ar[r,"{\int_{S_1}}"] &
     H^3(\Bdot \Gamma,\Z(1)) \\
     H^2(\Bdot\R,\Omega^1) \ar[r,"q^\ast"] \ar[u,"\simeq" sloped] &
     H^2(\Gamma \backslash S^1, \Omega^1) \ar[r,"{\int_{S_1}}"] \ar[u] &
     H^2(\Bdot \Gamma,\Omega^0) \ar[u]
 \end{tikzcd}
 \end{equation}
 Commutativity of the left-hand square expresses naturality of the 
 pullback under a change of coefficients. The right-hand square commutes by \cref{fibcomm}.

 We interpret the resulting class as the cohomology class of a central extension by
 postcomposing with the isomorphism $H^3(\Bdot \Gamma, \Z(1)) \to H^2(\Bdot \Gamma, \underline\T)$ 
 from \cref{lem:Tn_equiv_Zn}.
 Computing the transgression to $H^2(\Bdot \Gamma,\underline\T)$ hence comprises of 
 picking a representing class in 
 $H^2(\Bdot\R,\Omega^1)$, transgressing to $H^2(\Bdot\Gamma,\Omega^0)$, and
 composing the result with the exponential map
 \begin{equation}
     \exp(2\pi i): \Omega^0 \to \Z(1)[1] \to \underline\T.
 \end{equation}

 \begin{rem}
     The discussion above shows that the transgression map factors
     through the exponential 
     $H^2(\Bdot\Gamma,\Omega^0) \to H^2(\Bdot\Gamma,\underline\T)$.
     There is an extension $\GpVir_\R$ of $\Gamma$ by $\R$, with cohomology class
     the image of the differential lift of $p_1$ in $H^2(\Bdot\Gamma,\Omega^0)$.
     The Virasoro group $\GpVir$ as we construct it is the exponential of $\GpVir_\R$:
     the two extensions fit into a diagram
     \begin{equation}
     \begin{tikzcd}
         \R \ar[r] \ar[d,"\exp"] & \GpVir_\R \ar[r] \ar[d] & \Gamma \ar[d,equal] \\
         \T \ar[r] & \GpVir \ar[r] & \Gamma.
     \end{tikzcd}
     \end{equation}
 \end{rem}

 The group $H^2(\Bdot\R, \Omega^1)$ classifies central extensions of sheaves of abelian Lie groups over $\Man$ 
 of the form
 \begin{equation}
     \Omega^1 \to E \to \underline\R.
 \end{equation}

 \begin{lem}
     $H^2(\Bdot\R, \Omega^1)$ is generated by the class of the cocycle
 	\begin{equation}
     \begin{aligned}
         \omega_{\hat{p}_1}: \underline\R \times \underline\R &\to \Omega^1 \\
         (x_1, x_2) &\mapsto x_2 \ud x_1.
     \end{aligned}
 	\end{equation}
 \end{lem}

 \begin{proof}
     The group $H^2(\Bdot\R, \Omega^1)$ is isomorphic to $\R$ by \cref{pullback_to_diff_forms} and \cref{GLn_off_diag}.
     The sheaves $\Omega^i$ are soft on manifolds \TODO: reference,
     so $H^\ast(\Bdot\R,\Omega^i)$ is computed by the simplicial complex $\Omega^i(\Bdot\R)$:
     \begin{equation}
     \label{omegaOfBdotG}
         \begin{tikzcd}
 	        \Omega^i(\point)  
 	        \ar[r,shift left=0.1em]  \ar[r,shift right=0.1em]  & \Omega^i(G) 
 	        \ar[r,shift left=0.2em]  \ar[r] \ar[r,shift right=0.2em] & \Omega^i(G\times G) 
 	        \ar[r,shift left=0.3em]  \ar[r,shift left=0.1em]
 	        \ar[r,shift right=0.1em] \ar[r,shift right=0.3em] &\Omega^i(G\times G\times G) \dots,
         \end{tikzcd}
     \end{equation}
     and $k$-cocyles are those $1$-forms $\omega \in \Omega^i(G^k)$, whose alternating pullback to 
     $G^{k+1}$ vanishes.
     For $i=1, k=2$, it is straightforward to check that the 1-form
     $(x_1, x_2) \mapsto x_2 \d x_1$ is a cocycle, but not a coboundary in this complex.
 \end{proof}

 \TODO: insert some signposting here about what's happening now?

 The proof of the following Proposition will take up the rest of this note:
 \begin{prop}
     The transgression map 
     $\int_{S_1} \circ \ q^\ast: H^2(\Bdot\R,\Omega^1) \to H^2(\Bdot\Gamma,\Omega^0)$ sends the 
     class of the cocycle $\omega_{\hat{p}_1}: \underline\R \times \underline\R \to \Omega^1$
     to that of the extension $\underline\R \to \GpVir_\R \to \Gamma$
     with representing cocycle \TODO: different name for cocycle
     \begin{align}
       \int_{S_1} q^\ast \omega_{\hat{p}_1} : \Gamma \times \Gamma &\to \underline\R \\
                     (\gamma_1,\gamma_2) &\mapsto -\int_{S^1} \log(\gamma_1'\circ\gamma_2) \ud(\log(\gamma_2))'.
     \end{align}
   
 \end{prop}

 \TODO: say that the main statement is a corollary of this Proposition


 To compute the transgression map $H^2(\Bdot\R,\Omega^1) \to H^2(\Bdot\Gamma,\Omega^0)$ explicitly, 
 we consider $\GFR$ as a bisimplicial manifold $\GFR_{\bullet,\bullet}$, with 
 $\GFR_{p,q} = \Gamma^p \times F \times G^q$:

 \begin{equation}
 \begin{tikzcd}
     &
 	\cdots
 	\ar[d,shift left=0.3em]  \ar[d,shift left=0.1em]
 	\ar[d,shift right=0.1em] \ar[d,shift right=0.3em] &
 	\cdots
 	\ar[d,shift left=0.3em]  \ar[d,shift left=0.1em]
 	\ar[d,shift right=0.1em] \ar[d,shift right=0.3em] &
 	\cdots
 	\ar[d,shift left=0.3em]  \ar[d,shift left=0.1em]
 	\ar[d,shift right=0.1em] \ar[d,shift right=0.3em] 
 	\\
     \cdots
 	\ar[r,shift left=0.3em]  \ar[r,shift left=0.1em]
 	\ar[r,shift right=0.1em] \ar[r,shift right=0.3em] &
 	\Gamma^{\times 2} \times F \times G^{\times 2}
 	\ar[d,shift left=0.2em]  \ar[d] \ar[d,shift right=0.2em]
 	\ar[r,shift left=0.2em]  \ar[r] \ar[r,shift right=0.2em] &
     \Gamma \times F \times G^{\times 2}
 	\ar[d,shift left=0.2em]  \ar[d] \ar[d,shift right=0.2em]
 	\ar[r,shift left=0.1em]  \ar[r,shift right=0.1em] &
 	F \times G^{\times 2}
 	\ar[d,shift left=0.2em]  \ar[d] \ar[d,shift right=0.2em]
 	\\
     \cdots
 	\ar[r,shift left=0.3em]  \ar[r,shift left=0.1em]
 	\ar[r,shift right=0.1em] \ar[r,shift right=0.3em] &
 	\Gamma^{\times 2} \times F \times G
 	\ar[d,shift left=0.1em]  \ar[d,shift right=0.1em]
 	\ar[r,shift left=0.2em]  \ar[r] \ar[r,shift right=0.2em] &
     \Gamma \times F \times G
 	\ar[d,shift left=0.1em]  \ar[d,shift right=0.1em]
 	\ar[r,shift left=0.1em]  \ar[r,shift right=0.1em] &
 	F \times G
 	\ar[d,shift left=0.1em]  \ar[d,shift right=0.1em]
 	\\
     \cdots
 	\ar[r,shift left=0.3em]  \ar[r,shift left=0.1em]
 	\ar[r,shift right=0.1em] \ar[r,shift right=0.3em] &
 	\Gamma^{\times 2} \times F
 	\ar[r,shift left=0.2em]  \ar[r] \ar[r,shift right=0.2em] &
     \Gamma \times F 
 	\ar[r,shift left=0.1em]  \ar[r,shift right=0.1em] &
 	F 
 \end{tikzcd}
 \end{equation}

 %continue here: talk about the other two models and the weak equivalence

 Here's the main lemma that we need:
 \begin{lem}\label{main_lemma}
 The class $(0,0, x_2 \ud x_1)$ and $(\alpha, 0, 0)$ are cohomologous in the double complex. That is, their difference 
 \begin{equation}
     (-\alpha, 0, x_2 \ud x_1) = d \beta
 \end{equation}
 where $\beta = (\log(v)\ud\log(\gamma'), x \ud\log(v))$ is a  $2$-form in the double complex, with
 $\log(v)\ud\log(\gamma') \in \Omega^1(\Gamma \times F)$ and $x\ud\log(v) \in \Omega^1(F \times G)$.
 \end{lem}
 Here's what it looks like in pictures:
 (\TODO: draw something that helps seeing what's happening.)
 We need to show that the horizontal and vertical differentials of the $log\ v \ d\ log \gamma'$ is $\alpha$ and $x\ log\ \gamma$, and the horizontal and vertical differentials of $x \ d\ log\ v$ is $x \log \gamma$ and $x_2 \ dx_1$. (\TODO: proof the lemma somewhere.). 


% \end{proof}


% The pretty vertical diagram
% https://q.uiver.app/?q=WzAsMTYsWzAsMl0sWzEsMl0sWzIsMiwiSF40KFxcQmRvdFxcUjtcXFIoMikpIl0sWzMsMl0sWzIsMCwiSF4yKFxcQmRvdFxcUjtcXE9tZWdhXjEpIl0sWzIsMSwiSF40KFxcQmRvdFxcUjtcXFooMikpIl0sWzIsMywiXFxTeW1eMihcXGZnXlxcdmVlKV5cXFIiXSxbMiw0LCJIXjIoXFxCZG90XFxSO1xcT21lZ2FeMikiXSxbMSwxXSxbMSwzXSxbMywwXSxbMyw0LCItXFxmcmFjezF9ezhcXHBpXjJ9XFx1ZCB4XzFcXHVkIHhfMiJdLFsxLDQsIi1cXGZyYWN7MX17OFxccGleMn1cXHVkIHhfMVxcdWQgeF8yIl0sWzEsMCwiLVxcZnJhY3sxfXs4XFxwaV4yfSB4XzFcXHVkIHhfMiJdLFszLDEsIlxcaGF0e3B9XzEiXSxbMywzLCItXFxmcmFjezF9ezhcXHBpXjJ9QV4yIl0sWzQsNSwiXFxwc2lfMSJdLFs1LDJdLFsyLDYsIlxcZXFyZWZ7Ym90dHNfdGhlb3JlbTJ9Il0sWzYsNywiXFxlcXJlZnsycV9ib3R0fSIsMCx7ImNvbG91ciI6WzAsNjAsNjBdfSxbMCw2MCw2MCwxXV0sWzQsNywiXFxkIiwyLHsib2Zmc2V0Ijo1LCJjdXJ2ZSI6NX1dLFsxMywxMiwiXFxkIiwyLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFsxNCwxNSwiIiwyLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFsxNSwxMSwiPyIsMCx7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fSxbMCw2MCw2MCwxXV1d
\begin{equation}
\label{omega1_to_omega2_big_diagram}
\begin{tikzcd}
	& {-\frac{1}{8\pi^2} x_1\ud x_2} & {H^2(\Bdot\R;\Omega^1)} & {} \\
	& {} & {H^4(\Bdot\R;\Z(2))} & {\hat{p}_1} \\
	{} & {} & {H^4(\Bdot\R;\R(2))} & {} \\
	& {} & {\Sym^2(\fR^\vee)^\R} & {-\frac{1}{8\pi^2}A^2} \\
	& {-\frac{1}{8\pi^2}\ud x_1\ud x_2} & {H^2(\Bdot\R;\Omega^2)} & {-\frac{1}{8\pi^2}\ud x_1\ud x_2}
	\arrow["{\iota}", from=1-3, to=2-3]
	\arrow[from=2-3, to=3-3]
	\arrow["{\eqref{botts_theorem2}}", from=3-3, to=4-3]
	\arrow["{\textcolor{black}{\eqref{2q_bott}}}", color={rgb,255:red,214;green,92;blue,92}, from=4-3, to=5-3]
	\arrow["\d"', shift right=8, curve={height=30pt}, from=1-3, to=5-3]
	\arrow["\d"', maps to, from=1-2, to=5-2]
	\arrow["\eqref{distinguishedlifts}", maps to, from=2-4, to=4-4]
	\arrow["{?}", color={rgb,255:red,214;green,92;blue,92}, maps to, from=4-4, to=5-4]
\end{tikzcd}
\end{equation}

% OUTTAKE FROM "Main Statement"
Using the model of $\BdotG$ as a simplicial manifold (see \cref{Bdot}) enables us to use the 
Čech-simplicial double complex (\TODO: reference Brylinski?) to compute the cohomology groups above.
This is further simplified by the fact that the sheaves $\Omega^i$ are soft on manifolds \TODO: reference,
which makes the Čech-direction of the complex redundant.
The cohomology classes $H^k(\BdotG,\Omega^i)$ are computed by the simplicial complex 
$\Omega^i(\BdotG)$:
\begin{equation}
\label{omegaOfBdotG}
    \begin{tikzcd}
	    \Omega^i(\point)  
	    \ar[r,shift left=0.1em]  \ar[r,shift right=0.1em]  & \Omega^i(G) 
	    \ar[r,shift left=0.2em]  \ar[r] \ar[r,shift right=0.2em] & \Omega^i(G\times G) 
	    \ar[r,shift left=0.3em]  \ar[r,shift left=0.1em]
	    \ar[r,shift right=0.1em] \ar[r,shift right=0.3em] &\Omega^i(G\times G\times G) \dots,
    \end{tikzcd}
\end{equation}
and $k$-cocyles are those $i$-forms $\omega \in \Omega^i(G^k)$, whose alternating pullback to 
$G^{k+1}$ vanishes.

\cref{GLn_off_diag} shows that the group of off-diagonal differential lifts of 
$p_1 = 0 \in H^4(\BdotG)$ to $H^4(\BdotG,\Z(2))$ is naturally identified with
${\Sym^2(\gl_1(\R))}^{\GL_1(\R)} \iso \R$.
In order to write down explicit differential forms, we pick a set of coordinates 
$(x_1,x_2,\ldots,x_n)$ on $G^n=R^n$.
\begin{lem}
    The lift of $p_1$ corresponding to the polynomial $p(x)=x^2$ in ${\Sym^2(\gl_1(\R))}^{\GL_1(\R)}$
    is represented by the differential form 
    \begin{equation}
        \omega_{\hat{p}_1} \coloneqq \mathrm{\TODO} \cdot x_2 \d x_1 \in \Omega^1(\R^2).
    \end{equation}
\end{lem}
\begin{proof}
    That $x_2 \d x_1$ is a cocycle may be shown by direct computation:
    its coboundary is the alternating sum over the pullback maps in
    the simplicial complex \ref{omegaOfBdotG}. 
    The factor is a \TODO - otherwise rephrase section above
\end{proof}





% LEON's bit in Main Statement
Let's set our coordinates straight: the coordinates on $\mb{R}$ is $x$, the coordinate on $F = \mb{R}^{>0} \times S^1$ is $v, \theta$, the coordinate on $\Gamma$ is $\gamma$. $x$ acts on $F$ as
\begin{equation}
    (v, \theta) \mapsto (e^x v, \theta)
\end{equation}
and $\gamma$ acts on $F$ as 
\begin{equation}
    (v, \theta) \mapsto (\gamma'(\theta) v, \gamma(\theta))
\end{equation}


First we find explicit cocycle representatives for the map 
\begin{equation}
    Sym^2(\mathfrak{g})^G \simeq H^2(\BdotG, \Omega^1) \to H^3(\BdotG, \underline\T(1))
\end{equation}
Recall that $\BdotG = */G$ has a simplicial presentation:
\begin{equation}
\begin{tikzcd}
	\point & 
	\ar[l,shift left=0.1em] \ar[l,shift right=0.1em]  G &
	\ar[l,shift left=0.2em] \ar[l] \ar[l,shift right=0.2em] G\times G &
	\ar[l,shift left=0.3em] \ar[l,shift left=0.1em]
	\ar[l,shift right=0.1em] \ar[l,shift right=0.3em] G\times G\times G \dots
\end{tikzcd}
\end{equation}
Since $\Omega^1$ is soft on manifolds, that is, it has no higher cohomology, the Čech complex 
\begin{equation}
    \bigoplus^i \Omega^i(G) \leftarrow \cdots
\end{equation}
(\TODO: actually write it out)
computes the cohomology group $H^*(\BdotG, \Omega^1)$.
The differential is $\sum_i (-1)^i d_i^*$.
That is, we get explicit cocycles. Let $\beta \in Sym^2(\mathfrak{g})^G$ be the bilinear pairing with $\beta(\partial_x, \partial) = 1$. We have its cocycle representatives:
\begin{lem}
\label{explicit_x2x1}
The generator $\beta$ is map to the cohomology class of the cocycle $ x_2 \ dx_1 \in \Omega^1(\R^2)$.
\end{lem}



(\TODO: Leon: proof this somewhere, I actually don't really know how it works, need to look back at the Mike's talk).

Now we pullback this cocyle to $\GFG$, to do this, we also need a compatible simplicial presentation on $\GFG$, given by viewing it as $(\Gamma \backslash F)$ quotient by $G$:
\begin{equation}
    \cdots \rightarrow (\Gamma \backslash F) \times \mb{R}^2 \rightarrow (\Gamma \backslash F) \times \mb{R}^1 \rightarrow  (\Gamma \backslash F).
\end{equation}
(\TODO: Make this diagram better)

We have a simplicial map $(\Gamma \backslash F) / \mb{R}_\bullet \rightarrow B\mb{R}_\bullet$, taking $\Gamma \backslash F$ to a single point. We get a map of Čech complexes, 
oulling back the Čech cocycle $x_2 \ dx_1 \in \Omega^1(\mb{R}^2)$, we get the class $x_2 dx_1 \in \Omega^1((\Gamma \backslash F) \times  \mb{R}^2)$.

However, what we really want is a simplicial cocyle with respect to simplicial presentation of $\Gamma$ acting on $F/\mb{R} = S^1$:
\begin{equation}
    \cdots \rightarrow \Gamma^2 \times  (F/\mb{R}) \rightarrow \Gamma \times (F/\mb{R}) \rightarrow  F/\mb{R}.
\end{equation}
Because this is a $S^1$ fibration over the standard simplicial presentation of $B\Gamma = pt/\Gamma$, and we know how to integrate differential cohomology class in this presentation.

So we are task with the following question: how can we move cocycles from one simplicial presentation to another? The answer is clear, make it a double complex and then move cocycles from the vertical to horizontal. 


Think about when we have two projective resolution and how we show that they give the same cohomology, we form a double complex then do spectral sequence horizontally and vertically. On $E_1$ page they give the chain complex for the two resolutions. This is exactly what is happening here, however, we don't just want to show that they compute the same cohomology, but rather actually want to compute the cocycles on the other side. To do this, we need to set up the double complex and add coboundary terms to move them around. 

Here's the bisimplicial object $\Gamma \backslash F / \mb{R}_{\bullet, \bullet}$:
(\TODO: have a diagram here.)
We consider the double complex associated to the sheaf $\Omega^1[1]$ (\TODO: $\Omega^1[-1]$?) and this bisimplicial object. The relevant class is colored in purple in the diagram above. In this double complex,  A degree cocycle $(\omega_1, \omega_2, \omega_3)$ with $\omega_1 \in \Omega^1(\Gamma^2 \times F)$, $\omega_2 \in \Omega^1(\Gamma \times F \times \mb{R})$, and $\omega_3 \in \Omega^1(F \times \mb{R}^2)$ satisfies the following conditions
\begin{align}
    \sum_i (-1)^i(d_i ^h)^* \omega_1 = 0 \\
    \sum_i (-1)^i(d_i ^h)^* \omega_2 = \sum_i (-1)^i(d_i ^v)^* \omega_1 \\
    \sum_i (-1)^i(d_i ^h)^* \omega_3 = \sum_i (-1)^i(d_i ^v)^* \omega_2 \\
    \sum_i (-1)^i(d_i ^v)^* \omega_3 = 0
\end{align}
$d^h_i, d^v_i$ are the horizontal and vertical maps.


Recall that we have the cocycle class $x_2 \ dx_1 \in \Omega^1((\Gamma \backslash F) \times  \mb{R}^2)$, this pullback to the cocycle $(0,0, x_2 \ dx_1)$ in the double complex.
What we want is a cocycle of the form $(\alpha, 0, 0)$, and this will necessary comes from a cocycle in from the horizontal simplicial presentation, thus something we can simply integrate!

Here's one such candidate class: 
\begin{equation}
    \alpha = log(\gamma_2'(\theta)) \ dlog(\gamma_1'(\gamma_2 (\theta))) \ d\theta \in \Omega^1(\Gamma^2 \times F)
\end{equation}
Of course this is pullback from $\Gamma^2 \times F/\mb{R} = \Gamma^2 \times S^1$ as it doesn't depend on $v$.
